A machine learning pipeline for automated insect monitoring

Climate change and other anthropogenic factors have led to a catastrophic decline in insects, endangering both biodiversity and the ecosystem services on which human society depends. Data on insect abundance, however, remains woefully inadequate. Camera traps, conventionally used for monitoring terrestrial vertebrates, are now being modified for insects, especially moths. We describe a complete, open-source machine learning-based software pipeline for automated monitoring of moths via camera traps, including object detection, moth/non-moth classification, fine-grained identification of moth species, and tracking individuals. We believe that our tools, which are already in use across three continents, represent the future of massively scalable data collection in entomology.

==> ami_data_companion.tex <==
Insect camera traps produce a large number of images to store and process and it is necessary to implement an efficient, standardised and scalable workflow to manage each step of the machine learning pipeline (\autoref{fig:ml_workflow}). We therefore developed a tool, the AMI Data Companion, an open-source software package (link omitted for anonymity) designed to assist researchers with these steps. (AMI stands for \textbf{A}utomated \textbf{M}onitoring of \textbf{I}nsects.)
 
The primary function of the AMI Data Companion is to run machine learning models on large batches of images from insect camera traps and collate the results. Data from field deployments of camera systems can be reviewed before processing takes place, for example, to confirm that the devices ran as scheduled. Images can be processed on demand or placed into a fault-tolerant queue for long-running operations. The choice of model is configurable for each operation (e.g.~object detection, tracking, species classification). The software provides a graphical interface that can be run on all major desktop operating systems, as well as a command-line interface that can be run on multiple server nodes in parallel.

% This could also go in the pathways to impact section
The desire to scale automated insect monitoring globally has also led us to develop an online version of the application (in progress). The AMI Web Platform (\autoref{fig:ami_data_companion}) is designed to address challenges in taxonomic alignment, access to compute infrastructure, the curation of training data, and the need to collaborate with experts from around the world. This will make it possible for researchers to focus on downstream questions such as ecosystem change, distribution shift, etc.

\begin{figure}[hbt]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{TCCML_NeurIPS_2023_Style_File/figures/ami-1.png}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{TCCML_NeurIPS_2023_Style_File/figures/ami-2.png}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{TCCML_NeurIPS_2023_Style_File/figures/ami-4.png}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{TCCML_NeurIPS_2023_Style_File/figures/ami-3.png}
    \end{subfigure}    
    \caption{A preview of the AMI Web Platform in development.}
    \label{fig:ami_data_companion}
\end{figure}
